QoS-Aware Scheduling in New Radio Using Deep Reinforcement Learning

Fifth-generation (5G) New Radio (NR) cellular networks support a wide range of new services, many of which require an application-specific quality of service (QoS), e.g. in terms of a guaranteed minimum bit-rate or a maximum tolerable delay. Therefore, scheduling multiple parallel data flows, each serving a unique application instance, is bound to become an even more challenging task compared to the previous generations. Leveraging recent advances in deep reinforcement learning, in this paper, we propose a QoS-Aware Deep Reinforcement learning Agent (QADRA) scheduler for NR networks. In contrast to state-of-the-art scheduling heuristics, the QADRA scheduler explicitly optimizes for the QoS satisfaction rate while simultaneously maximizing the network performance. Moreover, we train our algorithm end-to-end on these objectives. We evaluate QADRA in a full scale, near-product, system level NR simulator and demonstrate a significant boost in network performance. In our particular evaluation scenario, the QADRA scheduler improves network throughput by 30% while simultaneously maintaining the QoS satisfaction rate of VoIP users served by the network, compared to state-of-the-art baselines.

==> comments.tex <==
- VoIP data flows, incorrect number? Experiments were actually run using 10 flows in either direction as RH generated 10 "phone calls", each requiring an uplink and downlink flow (or each requiring 20 "phone talkers" (:p), not sure on which interpretation is correct, can a radio flow serve both up and downlink or must these be separated into two? irrelevant for paper but still interested..)
    - see below

- Starvation plot, fix x label to say number of VoIP radio flows
    - Might have to updated ticks (see above!)
    - Simpler fix
    
- Radio flows vs. data flows?
    - Figs show radio flow atm, needs fixing if data flow is preferred
    - Switch to data flows
    
- Cell throughput vs. full buffer throughput
    - current formulation of reward function (updated!) suggests we optimize the throughput of full buffer throughput rather than cell throughput, which I suppose is the goal but not exactly how the simulations were run -- although these two values should be almost exactly identical.
    - Refer back to fig 2

- More related work?

- Need to check the references, especially the reviews... Text has changed a bit here and there so references might not be up to date everywhere.

- Claim QoS improved by 40\% because number of delayed packets are reduced by 30\% (1/0.7 approx 1.4...), okay or too far-fetched? :)
    - skip 40\% improve, claim improved only. drop rate reduced by 30\% (!!!)

- Document is now 7 pages
    - Could combine Figs. 5 \& 6, but will most likely cause a lot of clutter...
    
- Result section very short

- Conclusion?

To dos before next week:
- Finish abstract (all)
- Introduction (mainly Euhanna & Soma ?)
- Change "radio flow" into "data flow"
    - in text (Jakob)
    - and in Figures 1 & 3 (Soma?)
- Work on paper length (all)
    - Combine Figs. 5 & 6 (Soma?). 
        - This one I (Jakob) cannot do since I don't have access to the .fig files.
    - Make things concise whereever you see... 
    - Consider only having one of Figs 1 and 3.
- Minor comments:
    - on the number of VoIP flows vs. users, let it remain users but indicate that each user requires two flows
    - skip 40\% improvement and push the 30\% reduction more, e.g. by relating to packet drops
    - rewards, keep cell throughput as reward and refer back to fig. 2
    - highlight throughput reward more
    - thesis reference..?
    
During next meeting
- Finalize abstract (try to go into overleaf and check if it has changed a few times during the week)
- With finalized abstract, test the EDAS registration

Move other RL algorithms to conclusion/discussion (the end!)

- Figures not centered
- Absolute priority should probably switch to round robin
- Move delay opt. to last in legend
- Colors?
- Add separate optimizations to table?

    
    
    
    
INTRODUCTION - Soma & Euhanna
- Reference to thesis!!! Highlight thesis   (if you find a nice way)
MODEL - Vidit, Jakob
DRL - Vidit, Jakob
Algorithm - Jakob, Euhanna
Experiments & results - Jakob, Vidit
- refer to discussion of thesis     (if you find a nice way more mandatory-ish)
Conclusion - Soma, Euhanna

Figures & table - Jakob, Soma as backup
- Absolute priority should probably switch to round robin
- Colors?
- Add separate optimizations to table?

Fix line spacing - 1.0 -> 0.96 Jakob
Go through references... Jakob





Jakob:
- Table include RR also??
- References
    - Thesis
    - Style
    
    
    
mention round robin as well
separate opt. mention degradation
add "infinite episode of small sequences"
"maintaining qos"?

==> figs/model/starvation-cdf.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/model/starvation-cdf/dl.eps}
        \caption{}
        \label{fig:starvation-cdf:downlink}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/model/starvation-cdf/ul.eps}
        \caption{}
        \label{fig:starvation-cdf:uplink}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/model/starvation-cdf/delay.eps}
        \caption{}
        \label{fig:starvation-cdf:delay}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/model/starvation-cdf/nrofAllReq.eps}
        \caption{}
        \label{fig:starvation-cdf:nrofAllReq}
    \end{subfigure}
    \caption{Starvation in practice. One full buffer download and ten VoiP users that are given priority, compared to a random policy. The \subref{fig:starvation-cdf:downlink}) downlink and \subref{fig:starvation-cdf:uplink}) uplink throughputs are considerably larger with the priority based scheduler. However, large \subref{fig:starvation-cdf:delay}) VoiP packet delays affecting VoiP quality are considerably reduced using a random policy as well as the \subref{fig:starvation-cdf:nrofAllReq}) number of allocation requests given to the scheduler.}
    \label{fig:starvation-cdf}
\end{figure}


==> figs/results/combined.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/results/combined/dl-combined.eps}
        \caption{}
        \label{fig:combined:dl}
    \end{subfigure}
    \quad\quad\quad
    \begin{subfigure}{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/results/combined/delay-combined.eps}
        \caption{}
        \label{fig:combined:delay}
    \end{subfigure}
    \caption{Cumulative distributions of a) downlink network throughput and b) VoIP packet delays using DQNs trained with varying preference vectors.}
    \label{fig:combined}
\end{figure}


==> figs/results/separate.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{figs/results/separate/dl.eps}
        \caption{}
        \label{fig:separate:dl}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{figs/results/separate/delay.eps}
        \caption{}
        \label{fig:separate:delay}
    \end{subfigure}
    \caption{Cumulative distributions of a) downlink network throughput and b) VoIP packet delays using a DQN trained to maximize throughput (tpt) or VoIP delay only.}
    \label{fig:separate}
\end{figure*}


==> sections/method/mdp.tex <==
\subsection{MDP formulation}
Given the basic idea of the algorithm, let us formalize the state space $\cal S$ and action space $\cal A$
Let us present the MDP formulation of our algorithm, i.e. the state space $\cal S$, action space $\cal A$, state transition function $T$, reward function $R$, and discount factor $\gamma\in [0,1)$. The discount factor can be chosen arbitrarily.

\paragraph{State space} At each step of the selection sort, the state is characterized by the current input list, $\cal X$, and the current output list, $L$. Thus, the state space, $\cal S$, is given by
\begin{equation}
    \mathcal{S} = \mathcal{S}_i\times\mathcal{S}_o,
\end{equation}
where $\mathcal{S}_i=\mathcal{S}_o$, denoting the state spaces of the input and output lists, respectively. With each list containing a varying number of radio flows, each characterized by a feature vector in $\cal R$, their state spaces can be denoted by
\begin{equation}
    \mathcal{S}_i=\mathcal{S}_o= \mathcal{R} \cup \mathcal{R}\times\mathcal{R}\cup \ldots
\end{equation}
Given a continuous feature space, $\cal R$, the state space is hence also continuous.

\paragraph{Action space} The action space, $\cal A$ is discrete. At each step, an integer in $[0, n]$, where $n$ is the size of the current input list, is chosen. The integer chosen denotes the index, in the current input list, of the radio flow to be appended to the output list.

\paragraph{State transition model} The transition likelihoods are given by
\begin{equation}
    T: \mathcal{S}\times\mathcal{S}\times\mathcal{A} \to [0, \infty).
\end{equation}
The transitions are mostly deterministic. Indeed, the next state will always be determined by moving one element of the input list to the output list. Furthermore, the element to be moved is fully determined by the action selected. However, within each sorting sequence, the final state transition is indeed stochastic, as the radio flows update between each TTI out of the schedulers control.

\paragraph{Reward function}
Finally, the reward function can be designed rather arbitrarily as well. Aiming to optimize QoS-satisfaction, reasonable choices include giving negative reward when QoS was not maintained and positive rewards during times where QoS was maintained. The only limitation imposed by the framework is that non-zero rewards may only be given at the end of each sort, as the final list must be processed by the FD scheduler. That is, all intermediate rewards are zero.

==> sections/results/combined.tex <==
\subsection{Combined optimization}
Next, we proceed by \emph{jointly} optimizing the two objectives, in other words maximizing cell throughput while simultaneously maximizing QoS of VoIP data flows, by choosing a preference vector lacking zeros. However, since the two reward functions, $r_{\text{fb}}$ and $r_{\text{VoIP}}$, are not normalized to one another, a specific preference vector does not provide any insight into the actual network behavior. Finding a good preference vector, therefore, reduces to a trial and error process.

Using preference vectors
\[
    \omega^T\in\{[10, 1], [10, 0.1], [10, 0.01]\},
\]
resulting behaviors are shown in Fig. \ref{fig:combined}. Compared to the two baseline algorithms, our algorithm is able to improve cell throughput and QoS of VoIP users \emph{simultaneously}. The relative performance improvement of the algorithm to the round robin using VoIP priority is given in Table \ref{tab:results:multi}, also highlighting the influence of the preference vector. Using $\vec{\omega}^T = [10, 0.1]$, network throughput was increased by approximately $20\%$ and VoIP delays reduced by almost $30\%$, in other words improving QoS by almost $40\%$.

==> sections/results/separate.tex <==
\subsection{Separate optimization}
Consider, first, the two objectives, throughput maximization and VoIP packet delay minimization, separately, i.e. we train one policy for each objective by choosing $\vec{\omega}=[1, 0]^T$ or $\vec{\omega}=[0, 1]^T$, respectively. In Fig. \ref{fig:separate}, the resulting (empirical) CDFs of cell downlink throughput and VoIP packet delays are shown for the two learned policies. It is evident that the learned policies do succeed in their respective tasks of either maximizing throughput or minimizing the amount of delayed VoIP packets. The results serve as a sanity check of the algorithm. Furthermore, the inherent trade-off is highlighted as maximization of cell throughput results in poor VoIP QoS, and vice-versa.
